Relative Bogomolov extensions

An algebraic extension K of the rationals has the Bogomolov property if the absolute logarithmic height of non-torsion points of K* is bounded away from 0. We define a relative extension L/K to be Bogomolov if this holds for points of L\K. We construct various examples of extensions which are and are not Bogomolov. We prove a ramification criterion for this property, and use it to show that such extensions can always be constructed if some rational prime has bounded ramification index in K, when K is Galois over Q.

==> rbbackground.tex <==
We briefly describe what is known on fields with the Bogomolov property in order to put our results properly in context.  Schinzel \cite{schnitzel} showed in 1973 that there is a positive lower bound on the height of totally real numbers, establishing (B) for the maximal totally real field $\QQ^{tr}$.  This can be described as an ``archimedean'' height estimate, and was generalized by Garza to the following result, which we will apply in our proof of Theorem \ref{finram}.
\begin{theorem}[Garza \cite{sgbound}]
Let $K$ be a number field of degree $d$ over $\QQ$ with $r$ real places and $r'$ complex places.  If $K = \QQ(\gamma)$, then  
\begin{equation}\label{sgform}
H(\gamma) \geq \left( 2^{-d/r} + \sqrt{1+4^{-d/r}} \right)^{\frac{r}{2d}}.
\end{equation}
\end{theorem}
Another common approach that has been used, for example in \cite{habegger}, for archimedean estimates is equidistribution....

One non-archimedean strategy originates in Amoroso and Dvornicich's paper \cite{amorosodvornicich2000}, where it is shown that (B) is enjoyed by the maximal abelian extension $\QQ^{ab}$ of $\QQ$, which was strengthened considerably in \cite{az1} and \cite{az2}.  Their strategy involves estimating how close an element in a Galois group is to the action of raising an element to a power, with respect to a place lying over some auxilliary prime.  This strategy is quite powerful and is also used in \cite{habegger}, the elliptic curve analogue of \cite{amorosodvornicich2000}, and in \cite{adz}, where it is summarized nicely by their Lemma 2.2.  The main theorem (Theorem 1.2) of the latter paper generalizes both the results on abelian extensions and \cite[Theorem 2]{bombierizannier}, which states that (B) is satisfied by a field having bounded local degrees above some rational prime.  

In our present efforts to prove that a relative extension $L/K$ is Bogomolov when $K$ may not satisfy (B), it is not clear that the Amoroso-Dvornicich technique can be used to produce any new results.  Instead we appeal to more classical bounds in terms of discriminants.  Our main tool is the lower bound \cite[Theorem 2]{silvermanlb}, due to Silverman.  This bound is written in notation more similar to ours in \cite[Section 3]{widmerN}, where the author uses it effectively to give examples of fields satisfying the closely related Northcott property, (N).  This stronger property, first defined along with (B) in \cite{bombierizannier},  is satisfied by a field $K$ if for any $T$ at most finitely points in $K$ have height at most $T$.  Silverman's inequality generalizes to the relative case a type of bound going back to the theorem \cite[Theorem 1]{mahler} of Mahler, which is exactly the lower bound used in \cite[Theorem 2]{bombierizannier}, where as mentioned before the authors exploit the existence of a bound on local degrees above some finite rational prime.  Our Theorem \ref{finram} has the related hypothesis of finite ramification above a prime -- for this theorem we also require an archimedean estimate coming from the above stated theorem of Garza.
